Super-Resolution on the Two-Dimensional Unit Sphere

We study the problem of recovering an atomic measure on the unit 2-sphere $\mathbb{S}^2$ given finitely many moments with respect to spherical harmonics. The analysis relies on the formulation of this problem as an optimization problem on the space of bounded Borel measures on $\mathbb{S}^2$ as it was considered by Y. de Castro & F. Gamboa and E. Cand\'es & C. Fernandez-Granda. We construct a dual certificate using a kernel given in an explicit form and make a concrete analysis of the interpolation problem. Numerical examples are provided and analyzed.

==> Cover_Letter.tex <==



Dear Editors:

Please find attached our paper " Recovery of atomic measures on the unit sphere" that we would like to
submit for publication in the Journal of 
.
Our work develops a 

We hope you will also find our paper interesting and illuminating, and look forward to hearing from
you.
Sincerely,
Alexander Belton, Dominique Guillot, Apoorva Khare, and Mihai Putinar.
